From Collective Adaptive Systems to Human Centric Computation and Back: Spatial Model Checking for Medical Imaging

Recent research on formal verification for Collective Adaptive Systems (CAS) pushed advancements in spatial and spatio-temporal model checking, and as a side result provided novel image analysis methodologies, rooted in logical methods for topological spaces. Medical Imaging (MI) is a field where such technologies show potential for ground-breaking innovation. In this position paper, we present a preliminary investigation centred on applications of spatial model checking to MI. The focus is shifted from pure logics to a mixture of logical, statistical and algorithmic approaches, driven by the logical nature intrinsic to the specification of the properties of interest in the field. As a result, novel operators are introduced, that could as well be brought back to the setting of CAS.

==> eptcsdata.tex <==
\providecommand{\firstpage}{81}
\providecommand{\publicationstatus}{M.H. ter Beek and M. Loreti (Eds.): Workshop on\\ 
FORmal methods for the quantitative Evaluation\\ 
of Collective Adaptive SysTems (FORECAST'16).\\
EPTCS 217, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.217.10}{10.4204/EPTCS.217.10}}
\pdfoutput=1

